Finding It at Another Side: A Viewpoint-Adapted Matching Encoder for Change Captioning

Change Captioning is a task that aims to describe the difference between images with natural language. Most existing methods treat this problem as a difference judgment without the existence of distractors, such as viewpoint changes. However, in practice, viewpoint changes happen often and can overwhelm the semantic difference to be described. In this paper, we propose a novel visual encoder to explicitly distinguish viewpoint changes from semantic changes in the change captioning task. Moreover, we further simulate the attention preference of humans and propose a novel reinforcement learning process to fine-tune the attention directly with language evaluation rewards. Extensive experimental results show that our method outperforms the state-of-the-art approaches by a large margin in both Spot-the-Diff and CLEVR-Change datasets.

==> intro.tex <==
\section{Introduction}
The real world is a complex dynamic system. Changes are ubiquitous and significant in our day-to-day life. As humans, we can infer the underlying information from the detected changes in the dynamic task environments. % by digging the implied knowledge from the available explicit information. 
For instance, a well-trained medical doctor can judge the development of a patient's condition better by comparing the CT images captured in different time steps in addition to locating the lesion.   





\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{imgs/img_intro5.png}
    \caption{
    Current change captioning methods can be influenced by the viewpoint change between image pairs, which results in generating wrong captions.
    To address this problem, we propose a novel framework that aims at explicitly separating viewpoint changes from semantic changes.
    }
    \label{fig:intro}
\end{figure}


In recent years, a great deal of research has been devoted to \textcolor{\gu}{detecting} changes in various image content~\cite{bruzzone2000automatic,wang2018getnet,alcantarilla2018street,daudt2018fully}, which typically require a model to figure out the differences between the corresponding images. However, most of them focus on the changes in terms of object classes without paying much attention to various attribute changes (e.g., color and size). 
Moreover, \emph{change detection} usually requires pixel-level densely labeled ground-truth data for training the model. Acquiring such labeled data is too time-consuming and labor-intensive, \textcolor{\gu}{some of which, such as} in medical image applications even require human experts for generating annotations.
In addition, current change detection methods usually assume that the differences occur in an ideal situation. However, in practice, changes such as illumination and viewpoint changes occur quite frequently, which \textcolor{\gu}{makes} the change detection task even more challenging.


As humans, we can describe the differences between images accurately, since we can identify the most significant changes in the scene and filter out tiny differences and irrelevant noise. Inspired by the research development from dense object detection to image captioning, which generates natural language descriptions (instead of object labels) to describe the salient information in an image, the \emph{change captioning task} has recently been proposed to depict the salient 
differences between images~\cite{park2019robust,jhamtani2018learning,oluwasanmi2019fully,oluwasanmi2019captionnet}. Arguably, captions describing the changes are more accessible (hence preferred) for users, compared to the map-based labels (e.g., pixel-level binary maps as change labels). 

Despite the progress, the existing change captioning methods cannot handle the viewpoint change properly~\cite{park2019robust}. As shown in Fig.~\ref{fig:intro}, the viewpoint change in the images can overwhelm the actual object change leading to incorrect captions. Handling viewpoint changes is more challenging as it requires the model to be agnostic of the changes in viewpoints from different angles, while being sensitive to other salient changes.   

Therefore, in this paper, following the prevailing architecture of a visual encoder plus a sentence decoder, we propose a novel viewpoint-agnostic image encoder, called Mirrored Viewpoint-Adapted Matching (\textcolor{\gu}{M-VAM}) encoder, for the change captioning task. Our main idea is to exhaustively measure the feature similarity across different regions in the two images so as to accurately predict the changed and unchanged regions in the feature space. The changed and unchanged regions are formulated as probability maps, which are  used to synthesize the changed and unchanged features. We further propose a \textcolor{\gu}{Reinforcement Attention Fine-tuning (RAF)} process to allow the model to explore other caption choices by perturbing the probability maps.  


Overall, the contributions of this work include:
\begin{itemize}
    \item We propose a novel \textcolor{\gu}{M-VAM} encoder that explicitly distinguishes semantic changes from the viewpoint changes by predicting the changed and unchanged regions in the feature space.
    \item We propose a RAF module that helps the model focus on the semantic change regions so as to generate better change captions.
    \item Our model outperforms the state-of-the-art change captioning methods by a large margin in both Spot-the-Diff and CLEVR-Change datasets. Extensive experimental results also show that our method produces more robust prediction results for the cases with viewpoint changes.
\end{itemize}

